Multiversion Conflict Notion for Transactional Memory Systems

In recent years, Software Transactional Memory systems (STMs) have garnered significant interest as an elegant alternative for addressing concurrency issues in memory. STM systems take optimistic approach. Multiple transactions are allowed to execute concurrently. On completion, each transaction is validated and if any inconsistency is observed it is aborted. Otherwise it is allowed to commit. In databases a class of histories called as conflict-serializability (CSR) based on the notion of conflicts have been identified, whose membership can be efficiently verified. As a result, CSR is the commonly used correctness criterion in databases. Similarly, using the notion of conflicts, a correctness criterion, conflict-opacity (co-opacity) which is a sub-class of can be designed whose membership can be verified in polynomial time. Using the verification mechanism, an efficient STM implementation can be designed that is permissive w.r.t co-opacity. By storing multiple versions for each transaction object, multi-version STMs provide more concurrency than single-version STMs. But the main drawback of co-opacity is that it does not admit histories that are uses multiple versions. This has motivated us to develop a new conflict notions for multi-version STMs. In this paper, we present a new conflict notion multi-version conflict. Using this conflict notion, we identify a new subclass of opacity (a popular correctness-criterion), mvc-opacity that admits multi-versioned histories and whose membership can be verified in polynomial time. We show that co-opacity is a proper subset of this class. The proposed conflict notion mv-conflict can be applied on non-sequential histories as well unlike traditional conflicts. Further, we believe that this conflict notion can be easily extended to other correctness-criterion as well.

==> algo.tex <==
\section{Outline of a STM System using Multiversion Conflicts}
\label{sec:algo}

Having developed a conflict definition that accommodates multiple versions, we will now use this \mvconflict{} for developing multi-version STM system. The main idea behind the algorithm is based on the notion serialization graph testing \cite{SatVid:2011:ICDCN, KuzSat:NI:ICDCN:2014} that was developed for databases \cite{WeiVoss:2002:Morg}. According to this idea, the STM system maintains a graph based on the \op{s} that have been executed so far. A new \op{} is allowed to execute only if it does not form a cycle in the graph.

But a few important questions arise about the implementation which is typical of any multi-version system: (a) how many version should the STM system store? (b) which version should a transaction read from?

The issues of online scheduling was analyzed in \secref{ols} which partly addresses the question of which version should a transaction read from. Since whichever version a transaction reads from can possibly cause another transaction to abort, in our implementation we have decided to read the closest available version that does not violate \mvop. Using these ideas, we have developed a new algorithm described in the following sub-section. 

To address the question on number of versions maintained, it was shown in \cite{Kumar+:MVTO:ICDCN:2014} that by not maintaining a limit on the number of versions, greater concurrency can be achieved. So, we do not keep any limit on the number of versions maintained in the STM system developed. But with this approach the number of version keep growing over time. So, a garbage collection strategy that removes the unwanted versions. 


\subsection{Pseudocode}
\label{subsec:pcode}



%The question of which version a transaction must read from, the question was partly analyzed in \secref{ols}.
%in case of multi-version systems was first analyzed in the context of database systems \cite{HadzPapad:AAMVCC:PODS:1985}. A transactional system (either Database or STM) must decide in a ``on the spot'' which version a transaction can read from based on the past history. But this on the spot decision can lead to unnecessary aborts of transactions. Consider a read \op{} of $T_i$ on $x$, $r_i(x)$. Suppose $T_i$ has the option of reading from multiple versions of $x$, say $v_1, ... v_k$. Let the STM system assigns $v_1$ to the $r_i(x)$. But at a later point in time, another transaction $T_j$ is aborted due to this read option. Transaction $T_j$ might not be aborted if $T_i$ read a different version say $v_2$ for $x$ instead of $v_1$. We illustrate this in later section.


\cmnt {

But a few important questions arise about the implementation which is typical of any multi-version system: (a) how many version should the STM system store? (b) which version should a transaction read from?

To address the question on number of versions maintained, it was shown in \cite{Kumar+:MVTO:ICDCN:2014} that by not maintaining a limit on the number of versions, greater concurrency can be achieved. So, we do not keep any limit on the number of versions maintained in the STM system developed. But we have devised a garbage collection strategy that removes the unwanted versions. 

The question of which version a transaction must read in case of multi-version systems was first analyzed in the context of database systems \cite{HadzPapad:AAMVCC:PODS:1985}. A transactional system (either Database or STM) must decide in a ``on the spot'' which version a transaction can read from based on the past history. But this on the spot decision can lead to unnecessary aborts of transactions. Consider a read \op{} of $T_i$ on $x$, $r_i(x)$. Suppose $T_i$ has the option of reading from multiple versions of $x$, say $v_1, ... v_k$. Let the STM system assigns $v_1$ to the $r_i(x)$. But at a later point in time, another transaction $T_j$ is aborted due to this read option. Transaction $T_j$ might not be aborted if $T_i$ read a different version say $v_2$ for $x$ instead of $v_1$. We illustrate this in later section.

This requirement of on the spot scheduling was termed as online schedulable (OLS) in databases literature \cite{PapadKanel:1984:MultVer:TDS, HadzPapad:AAMVCC:PODS:1985}. We show that due online scheduling, STM systems can not be permissive w.r.t \mvopty{} due to multiple versions present. This is illustrated in the following sub-section.

\subsection{Result obtained so far}
As a part of this research, we developed a MVC(Multiversion Conflict) algorithm which satisfies Conflict Opacity. This algorithm has developed for Multiversion STMs based on multiversion conflicts.

\textbf {MVC algorithm works as follows:-}
\begin{enumerate}
\item \textbf{Read rule:} An operation $r_i(x)$ can read from the most previous closest write. If addition of Commit-read conflict edge to the $MVCG(H)$ will form a cycle then it will read from the next-previous closest write and so on. It ensures read always succeeds. In other words, any read operation can reads from at least one of the available version that will never form a cycle in the graph.
\item \textbf{Write rule:} Transaction $T_i$ writes into local memory.
\item \textbf{Commit rule:} If it is a read-only transaction, then always commits. If it is not, then for every try-to-commit, if it is founded conflict and the corresponding conflict edge will form a cycle in the graph then try-to-commit operation will be rejected and transaction will abort otherwise succeeds.

\end{enumerate}

\subsection{Data Structures}

\subsection{Pseudo code}

\subsection{Correctness of MCN}

}
